Unsynchronized Decentralized Q-Learning: Two Timescale Analysis By Persistence

Non-stationarity is a fundamental challenge in multi-agent reinforcement learning (MARL), where agents update their behaviour as they learn. Many theoretical advances in MARL avoid the challenge of non-stationarity by coordinating the policy updates of agents in various ways, including synchronizing times at which agents are allowed to revise their policies. Synchronization enables analysis of many MARL algorithms via multi-timescale methods, but such synchronization is infeasible in many decentralized applications. In this paper, we study an unsynchronized variant of the decentralized Q-learning algorithm, a recent MARL algorithm for stochastic games. We provide sufficient conditions under which the unsynchronized algorithm drives play to equilibrium with high probability. Our solution utilizes constant learning rates in the Q-factor update, which we show to be critical for relaxing the synchronization assumptions of earlier work. Our analysis also applies to unsynchronized generalizations of a number of other algorithms from the regret testing tradition, whose performance is analyzed by multi-timescale methods that study Markov chains obtained via policy update dynamics. This work extends the applicability of the decentralized Q-learning algorithm and its relatives to settings in which parameters are selected in an independent manner, and tames non-stationarity without imposing the coordination assumptions of prior work.

==> 2024-03-21-algo_sec_d1.tex <==
\section{Unsynchronized Decentralized Q-Learning} \label{sec:learning-algorithms}

In this section, we present Algorithm~\ref{algo:main}, an unsynchronized variant of the decentralized Q-learning of \cite{arslan2017decentralized}. Unlike in the original decentralized Q-learning algorithm, Algorithm~\ref{algo:main} allows for the sequence of exploration phase lengths $\{T^i_k \}_{k \geq 0}$ vary by agent. \blue{Although this change introduces non-stationarity and thus complicates the analysis significantly, we note that the algorithm itself is no more intricate than that of \cite{arslan2017decentralized}.} \red{try to reformat and bring algo before \S4.1 (primitive RVs).}

\begin{algorithm2e}[h] 

%	 \scriptsize % to make it real small
	\SetAlgoLined
	\DontPrintSemicolon
	\SetKw{Receive}{Receive}
	\SetKw{Reset}{Reset}
	\SetKw{parameters}{Set Parameters}
	\SetKw{initialize}{Initialize}
 
	\SetKwBlock{For}{for}{end}
	
	\parameters \; 
	\Indp 
%	$\qq^i \subset \rr^{\xx \times \uu^i }$: a compact set\; 
	$\{ T^i_k \}_{k \geq 0}$: a sequence in $\nn$ of learning phase lengths \; 
	\vspace{1pt}
		\Indp
		Put $t^i_0 = 0$ and $t^i_{k+1} = t^i_k + T^i_k$ for all $k \geq 0$.  \; 
		\Indm
	\vspace{1pt}
	$\rho^i \in (0,1)$: experimentation probability \; 
	$\lambda^i \in (0,1)$: inertia during policy update \; 
	$\delta^i\in(0,\infty)$: tolerance level for sub-optimality \; 
	$\alpha^i \in (0,1)$: step-size parameter (also called the learning rate) \; 
	\Indm
	\BlankLine
	
 	\initialize  $\pi_0^i \in \IndividualPolicySet^i_{SD}$, $\widehat{Q}_0^i \in \rr^{ \xx \times \uu^i }  $ (arbitrary) \\ 

	
	\For($k \geq 0$ ($k^{th}$ exploration phase for agent $i$ {)}){ %i  had to put { and } around ) because otherwise it misunderstands it as ending the for-loops condition.
		\For( $t = t_k^i, t_k^i +1, \dots, t^i_{k+1} - 1$)  %\tcp*[f]{Policy evaluation loop} )
		{
			Observe $x_t$ \; 
			Select $u^i_t = \begin{cases} \pi^i_k ( x_t ) , &\text{w.p. } 1 - \rho^i  \\ u^i \sim \uniform(\uu^i), &\text{w.p. } \rho^i \end{cases} 	$  \;
			
			Observe cost $c^i_t := c( x_t, \bu_t )$, state $x_{t+1}$ \;
			
			Put $\Delta^i_t = c^i_t + \discount^i \min_{a^i} \widehat{Q}^i_t ( x_{t+1}, a^i )$ \;

			\vspace{3pt}
			$\widehat{Q}^i_{t+1} (x_t  ,u_t^i)  =  (1-\alpha^i ) \widehat{Q}_t^i(   x_t  ,u_t^i) + \alpha^i  \Delta^i_t$  \;
			
			$\widehat{Q}_{t+1}^i(x,u^i) =  \widehat{Q}^i_t (x,u^i)$,   for all $(x,u^i)\not=(x_t,u_t^i)$\;

		}
		\vspace{3pt}  % toggle this when shrinking algorithm font size in pre-amble. when size = \small, use -3 or so, when not shrunk, use +6pt
		
		\BlankLine 
	
		\If { $\pi^i_k \in \widehat{\BR}^i_{ \delta^i} ( \widehat{Q}^i_{t^i_{k+1}} )$,}{ $\pi^i_{k+1} \leftarrow \pi^i_k$ }
		%\Else($i$ not satisfied){}
		\Else( ){$\pi^i_{k+1} \leftarrow \begin{cases} \pi^i_k , &\text{w.p. } \lambda^i \\ \pi^i \in    \widehat{\BR}^i_{  \delta^i} ( \widehat{Q}^i_{t^i_{k+1}} )  , &\text{w.p. } 1 - \lambda^i \end{cases} $ }
 

%		\If { $\widehat{J}^i_{t_{k+1}} ( y ) \leq \min_{a^i} \widehat{Q}^i_{t_{k+1}} ( y , a^i )  + \epsilon + d^i$ $\forall y \in \yy$,}{ $\pi^i_{k+1} = \pi^i_k$ }
%		%\Else($i$ not satisfied){}
%		\Else( ){$\pi^i_{k+1} \sim (1- e^i) \delta_{\pi^i_k} + e^i \uniform ( \Pi^i) $ ) }
 
	}
	
	\caption{Unsynchronized Decentralized Q-Learning} \label{algo:main}
\end{algorithm2e}




\subsection{Primitive Random Variables} \label{ss:primitive-random-variables}

We now introduce several collections of \emph{primitive} random variables that will be used in describing the assumptions and implementation of Algorithm~\ref{algo:main}. For any player $i \in \NN$ and $t \geq 0$, we define the following random variables:

\begin{itemize}
	
	\setlength \itemsep{1.5pt}
	
	\item $\{ W_t \}_{t \geq 0}$ is an identically distributed, $[0,1]$-valued stochastic process. For some $f : \xx \times \bU \times [0,1] \to \xx$, state transitions are driven by %the exogenous noise process 
	$\{ W_t   \}_{t \geq 0}$ via $f$: 
%		\begin{align*}
%			&\P ( x_{t+1} = s' | x_t = s, \bu_t = \ba ) = P ( s' | s, \ba )  \\
%		 = 	&\P \left( W_t  \in \{ w : f( s, \ba, w ) = s' \} \right),  
%		\end{align*}
		\begin{align*}
			\P ( x_{t+1} = s' | x_t = s, \bu_t = \ba ) = \P \left( W_t  \in \{ w : f( s, \ba, w ) = s' \} \right), 
		\end{align*}
	
	for any $(s,\ba, s') \in \xx \times \bU \times \xx$ and $ t \geq 0$;
		
	\item $\tilde{u}^i_t \sim \uniform( \uu^i )$;
	
	\item $\tilde{\rho}^i_t \sim \uniform( [0,1])$;
	
	\item $\tilde{\lambda}^i_t \sim \uniform( [0,1] )$;
	
	\item For non-empty $B^i \subseteq \IndividualPolicySet^i_{SD}$, $\tilde{\pi}^i_t ( B^i ) \sim \uniform ( B^i )$;
	
	\item $T^i_t$ is an $\nn$-valued random variable, elaborated below. 
\end{itemize}


\begin{assumption} \label{assumption:primitive-random-variables}
The collection of primitive random variables $\VV_1 \cup \VV_2$ is mutually independent, where 
\begin{align*}
\VV_1 &:= \bigcup_{i \in \NN, t \geq 0 } \left\{ W_t, \tilde{\rho}^i_t, \tilde{u}^i_t, \tilde{\lambda}^i_t, T^i_t \right\},    				\\
\VV_2 &:= \bigcup_{i \in \NN, t \geq 0} \left\{ \tilde{\pi}^i_t ( B^i ) : B^i \subseteq \IndividualPolicySet^i_{SD}, B^i \not= \varnothing \right\}. 
\end{align*}
\end{assumption}


\noindent \textbf{Remark:} With the exception of the exploration phase lengths $\{ T^i_k \}_{ \in \NN, k \geq 0}$, the random variables in $\VV_1 \cup \VV_2$ are primitive random variable that do not depend on any player's choice of hyperparameters or on the history of play of the game.
%The random variables in $\VV_1 \cup \VV_2$ are primitive random variables that, with the exception of exploration phase lengths $\{ T^i_k \}_{i \in \NN, k \geq 0}$, do not depend on any player's choice of hyperparameters.  
The exploration phase lengths are hyperparameters that we allow to be randomly selected at the outset of play.
We also note that the primitive random variables $\{ \tilde{u}^i_t : i \in \NN, t \geq 0\}$ should not be conflated with the action process $\{ u^i_t : i \in \NN, t \geq 0\}$, which depends on the sample path and is not a collection of primitive random variables. 



\subsection{Assumptions}

In order to state our main result, \Cref{theorem:main}, we now impose some assumptions on the underlying game $\GG$ and on the hyperparameters chosen by each player. \red{replace $\bu_t$ by $\ba_t$ and $\ba_t$ by ${\ba}^{\prime}_t$ below.}


\begin{assumption} \label{assumption:state-visitation} 
For any pair $(s, s') \in \xx \times \xx$, there exists $H = H( s, s' ) \in \nn$ and a sequence of joint actions \emph{$\ba_0, \dots, \ba_H \in \bU$} such that 
\[
\P ( x_{H+1} = s' | x_0 = s, \text{\emph{$\bu_0 = \ba_0, \dots, \bu_H = \ba_H$}} ) > 0 .
\]
\end{assumption}

\vspace{5pt}
\Cref{assumption:state-visitation} requires that the state process can be driven from any initial state to any other state in finitely many steps, provided a suitable selection of joint actions is made. This is a rather weak assumption on the underlying transition kernel $P$, and is quite standard in the theory of MARL (c.f. \cite[Assumption 4.1, Case iv]{ozdaglar2021independent}).


Our next assumption restricts the hyperparameter selections in Algorithm~\ref{algo:main}. Let $\bar{\delta} := \min \left( \mathfrak{A} \setminus \{ 0 \} \right)$, where
\begin{align*}
 \mathfrak{A}  :=  {\big \{}  &  {\big \vert} Q^{*i}_{ \bpi^{-i}} ( s, a^i_1 ) - Q^{*i}_{\bpi^{-i}} ( s, a^i_2)  {\big \vert } :   i \in \NN, \bpi^{-i} \in \JointPolicySet^{-i}_{SD}, s \in \xx,  a^i_1, a^i_2 \in \uu^i {\big \} } .
 \end{align*}

The quantity $\bar{\delta}$, defined originally by \cite{arslan2017decentralized} and recalled above, is the minimum \textit{non-zero} separation between two optimal Q-factors with matching states, minimized over all agents $i \in \NN$ and over all policies $\bpi^{-i} \in \JointPolicySet^{-i}_{SD}$.


For any baseline policy $\bpi \in \JointPolicySet_{SD}$ and fixed experimentation parameters $\{ \rho^i \}_{i \in \NN}$, we use the notation $\hat{\bpi} \in \JointPolicySet_{S}$ to denote a corresponding behaviour policy, which is stationary but not deterministic. When using $\hat{\pi}^i$, agent $i \in \NN$ follows $\pi^i$ with probability $1- \rho^i$ and mixes uniformly over $\uu^i$ with probability $\rho^i$. It was previously shown in \cite[Lemma B3]{arslan2017decentralized} that the optimal Q-factors for these two environments will be close provided $\rho^i$ is sufficiently small for all $i \in \NN$. In particular, there exists $\bar{\rho} > 0$ such that if $\rho^i \in (0, \bar{\rho})$ $\forall i \in \NN$, then 
\begin{equation}
\| Q^{*j}_{\bpi^{-j}} - Q^{*j}_{\hat{\bpi}^{-j}} \|_{\infty} < \frac{ \min_{i \in \NN} \min \{ \delta^i, \bar{\delta} - \delta^i \}}{4}  , \: \forall j \in \NN, \bpi^{-j} \in \JointPolicySet^{-j}_{SD} .   \label{eq:hat-policy}
\end{equation}

\vspace{2.5pt} 

\begin{assumption} \label{assumption:rho-delta}
For all $i \in \NN$, $\delta^i \in ( 0, \bar{\delta} )$ and $\rho^i \in ( 0, \bar{\rho} )$. 
\end{assumption}

\vspace{2.5pt} 

We require that $\delta^i$, player $i$'s tolerance for sub-optimality in its Q-factor, is positive to account for noise in its learning iterates, as exact convergence is unreasonably demanding during a truncated learning phase. On the other hand, the tolerance parameter $\delta^i$ is upper bounded so as to exclude truly suboptimal policies from consideration in an estimated best-response set. 

The second part of \Cref{assumption:rho-delta} concerns the experimentation parameter $\rho^i$. We assume that $\rho^i > 0$ so that player $i$ can explore all of its actions and accurately learn its Q-factors in the limit. This experimentation parameter $\rho^i$ must be kept small, however, so player $i$'s behaviour policy closely approximates its baseline policy.  \Cref{assumption:rho-delta} appears as Assumption~2 in \cite{arslan2017decentralized}.

\vspace{2.5pt} 


\begin{assumption} \label{assumption:exploration-phases}
There exists integers $R, T \in \nn$ such that  
\[
\P \left( \cap_{i \in \NN, k \geq 0} \left\{ T^i_k \in [T, RT] \right\} \right) = 1 . 
\]
\end{assumption}

\

\Cref{assumption:exploration-phases} requires that each agent spends a long time learning during any given exploration phase ($T^i_k \geq T$ almost surely for any player $i$ during any exploration phase $k$). The second part of \Cref{assumption:exploration-phases}, that $T^i_k \leq RT$ almost surely for all $i, k$, is assumed in order to control the relative frequency at which different agents update their policies.This is done to avoid the potentially problematic regime in which some agents update their policies an enormous number of times and repeatedly disrupt the learning of another agent who uses long exploration phase lengths.


%\vspace{5pt}
%
%
%\by{For clarity, it might be beneficial to break the technical exposition into two parts: 
%\begin{enumerate}
%	\item deterministic $\{T^i_k \}_{i, k}$ and the simpler proof. 
%	\item primitive random variable $\{T^i_k \}_{i, k}$ and the full proof. 
%\end{enumerate}
%}

\vspace{5pt}


When all players use Algorithm~\ref{algo:main}, we view the resulting sequence of policies $\{ \pi^i_k \}_{k \geq 0}$ as player $i$'s \emph{baseline} policy process, where $\pi^i_k$ is player $i$'s baseline policy during $[t^i_k, t^i_{k+1})$, player $i$'s $k^{th}$ exploration phase. This policy process $\{ \pi^i_k \}_{k \geq 0}$ is indexed on the coarser timescale of exploration phases. For ease of reference, we also introduce a sequence of baseline policies indexed by the finer timescale of stage games. For $t \geq 0$ with $t \in [t^i_k, t^i_{k+1} )$, we let $\phi^i_t := \pi^i_k$ denote player $i$'s baseline policy during the stage game at time $t$. The baseline joint policy at stage game $t$ is then denoted $\bphi_t = ( \phi^i_t )_{i \in \NN}$. Furthermore, we refer to the collection of Q-factor step-size parameters $\{ \alpha^i \}_{i \in \NN} $ as $\balpha \in (0,1)^N$.  

\vspace{5pt}

\begin{theorem} \label{theorem:main}
Let $\GG$ be a weakly acyclic game and suppose each player $i \in \NN$ uses Algorithm~\ref{algo:main} to play $\GG$. Suppose Assumptions~\ref{assumption:primitive-random-variables}--\ref{assumption:exploration-phases} hold, and let $\epsilon > 0$. There exists $\bar{\alpha}_{\epsilon} > 0 $ and a function $\bar{T}_{\epsilon} : (0,1)^N \times \nn \to \nn$ such that if 
\[
\max_{i \in \NN} \alpha^i < \bar{\alpha}_{\epsilon} , \text{ and } T \geq \bar{T}_{\epsilon} ( \balpha, R ) ,
\]
then $ \P ( \bphi_t \in \eq[0]_{SD} ) \geq 1 - \epsilon,$ for all sufficiently large $t \in \nn$. 
\end{theorem}


%\vspace{5pt}

\ 

In words, \Cref{theorem:main} says the following: if the relative frequency of policy update times of different players is controlled by some ratio $R$, if players use sufficiently small learning rates $\balpha$, and if the lower bound $T$ on each player's exploration phase length is sufficiently long relative to both the learning rates $\balpha$ as well as the ratio parameter $R$, then play will be driven to equilibrium with high probability.

\vspace{5pt}

As we will see, the interdependence of the various parameters---$R, \balpha,$ and $T$---is significant in the analysis to follow. % With the exception of a section for a simulation study, the remainder of this paper is devoted to proving \Cref{theorem:main} and discussing insights from the analysis of the proof. 


==> proof-overview.tex <==
\section{Proof Overview}   \label{sec:proof-outline}
\blue{
As we will see in \Cref{sec:proof}, the proof of \Cref{theorem:main} is somewhat intricate. For this reason, we now offer an outline of the proof to facilitate its reading. To further assist the reader in understanding the proof, a description of the proof under the synchronization assumption is given in Appendix~\ref{appendix:?} and a discussion on technical complications that arise when synchronization is relaxed is provided in Appendix~\ref{appendix:??}. 
}

\subsection{High-Level Overview}

\blue{
The proof of \Cref{theorem:main} involves three major steps. First, we introduce a sequence of equilibrium events, $\{ B_k \}_{k \geq 0}$, defined in terms of a suitably defined sequence of time intervals $\{ [ \tau^{\min}_k, \tau^{\max}_k ] \}_{k \geq 0}$, to be elaborated in the sequel. For $k \geq 0$, we put
\[
B_k := \left\{ \bphi_t =  \bphi_{\tau^{\min}_k} \in \eq_{SD}: t = \tau^{\min}_k + 1, \cdots, \tau^{\max}_k \right\} .
\]

In words, $B_k$ is the event in which the baseline policy did not change during the interval $[\tau^{\min}_k , \tau^{\max}_k]$ and moreover the baseline policy was an equilibrium during this time.
}

\blue{
Second, for a particular integer $L < \infty$ (defined in the text preceding \Cref{lemma:stay-at-equilibrium}), we argue in \Cref{lemma:stay-at-equilibrium} that we can control and lower bound the probability of remaining at the equilibrium event for $L$ steps: that is, $\P ( B_{k+L} | B_k ) $ can be made arbitrarily large by suitable selection of algorithm parameters. The proof of \Cref{lemma:stay-at-equilibrium} uses convergence properties of Q-learning iterates (\Cref{lemma:primitive-random-variables-lead-to-Q-convergence}) and requires careful arguments about conditional probabilities, since conditioning on the event $B_k$ carries confounding information about the state-action trajectory from both \emph{before and after} time $\tau^{\min}_k$ and precludes simple analysis that disconnects the future evolution of Q-learning estimates from the history of the system before time $\tau^{\min}_k$. Consequently, the analysis is somewhat delicate, and is worded in terms of primitive random variables, which offers a path around the confounding effect of conditioning on $B_k$.}

\blue{
Third, we argue in \Cref{lemma:go-to-equilibrium} that the probability of driving play to this equilibrium event in $L$ time steps can be lower bounded by a positive constant.  After this is achieved, one can then explicitly lower bound $\P ( B_{k+mL} )$ for suitably large $m$, as in \cite{arslan2017decentralized} and \cite{yongacoglu2023satisficing}.
}





\subsection{The Proof Under Synchronization} \label{ss:proof-with-synchronization}
\blue{To help the reader build intuition and to explain why certain analytical devices were needed in the proof of \Cref{theorem:main}, we now describe the proof in the simpler setting where players are synchronized with one another, as studied in \cite{arslan2017decentralized}. }

\blue{
In the synchronized variant of the algorithm, we have $T^i_k = T^j_k =T_k$ for any agents $i, j \in \NN$ and $k \geq 0$. Agents always begin and end their exploration phases in synch. Crucially, no agent ever switches its policy while another agent is actively learning its Q-factors. As a result, each agent faces an MDP during each exploration phase, and one can study the convergence of Q-factors using single-agent theory. In particular, when player $i$ employs suitably \emph{decreasing} step-sizes, one has that $\widehat{Q}^i_t \to Q^{*i}_{\bpi^{-i}_k}$, as $T_k  \to \infty$. 
}

\blue{
When analyzing the algorithm under the assumption that players are synchronized, one defines $\tau^{\min}_k = \tau^{\max}_k = t_k$, the stage game time marking the beginning of the $k^{th}$ shared exploration phase. With these choices of $\tau^{\min}_k$ and $\tau^{\max}_k$, the equilibrium event $B_k$ is equivalent to $\{ \bpi_k \in \eq_{SD} \}$. 
}

\blue{
Importantly, in the synchronized case, one is guaranteed that the joint policy is fixed at $\bpi_k$ throughout the interval $[t_k , t_{k+1} )$. Thus, each player $i$ spends $T_k$ stages learning against the policy $\bphi^{-i}_{\tau^{\max}_k} = \bpi^{-i}_k$. Furthermore, the Q-factors involved in policy updating at time $t_{k+1}$ are conditionally independent of the system's history before time $t_k$, given the state $x_{t_k}$, the joint policy $\bpi_k$, and the initial values of each agent's Q-factors at time $t_k$. This conditional independence fact is helpful in the synchronized setting, since conditioning on $B_k$ effectively decouples the history of the system (before $\tau^{\min}_k$) from its consequent evolution (after $\tau^{\min}_k$) , and allows one to analyze relevant quantities in isolation and obtain clean, uniform bounds on the convergence of Q-learning iterates. 
}

\blue{
In the synchronized setting, one can explicitly and uniformly lower bound the conditional probability $\P ( B_{k+L} | B^c_k ) $ by a quantity $\hat{p}_{\min} > 0$. This is done using weak acyclicity of the game $\GG$ and conditioning on an event where players learn their Q-factors approximately correctly in each of the exploration phases $k, k +1, \dots, k+L$, where the probability of the latter event can be controlled by taking exploration phase lengths $T_k, \dots, T_{k+L}$ to be suitably large.  
}

\blue{
At equilibrium, if players recover their optimal Q-functions, then they will opt to remain with their current policies.  Under synchronization, the probability of (approximately) recovering optimal Q-functions can be controlled directly by taking the \emph{shared} exploration phase lengths $\{ T_k \}_{k \geq 0}$ to be large. Thus, showing that $\P ( B_{k+L} | B_k )$ can be made large relative to $\hat{p}_{\min}$, is straightforward in the synchronized setting. 
}



\subsection{Challenges in the Unsynchronized Case}  

\blue{In the unsynchronized setting, where $T^i_k \not= T^j_k$ is allowed, we observe that the preceding definitions of $\tau^{\min}_k$ and $\tau^{\max}_k$ are not meaningful, since there is no shared $k^{th}$ exploration phase. Consequently, a new definition of the equilibrium event $B_k$ is required. The discussion below surveys some considerations that arise when selecting a suitable alternative definition for one's equilibrium events.
}

\subsubsection{Equilibrium Events and Conditional Probabilities}


%%%				Take 1.... revised below.
%%%
%%\blue{
%%Any useful definition of $\{ B_k \}_{k \geq 0}$ must be \emph{self-reinforcing}, in the sense that $\P ( B_{k+L} | B_k )$ should be controllable by appropriate choice of hyperparameters. In particular, the most natural way to approach this is by attempting to control the conditional probability that players approximately recover their equilibrium Q-functions given that the equilibrium event occurred. Since each player's Q-factors are constructed using historical feedback data, one must account for the recent history of play when analyzing Q-iterates in the unsynchronized setting. For illustration, let us consider player $i$'s $m^{th}$ exploration phase, and let us suppose that $t^i_{m+1} \in ( \tau^{\min}_k, \tau^{\max}_k ]$. In its $m^{th}$ exploration phase, player $i$ learns from time $t^i_m$ to time $t^i_{m+1} = t^i_m + T^i_m$. During this interval, player $i$'s counterparts may have switched policies several times. Thus, if one wishes to ensure that player $i$'s Q-factor estimates at time $t^i_{m+1}$ accurately reflect the prevailing environment, which is determined by $\bphi^{-i}_{t^i_{m+1}}$, then the conditioning event $B_k$ should guarantee that player $i$ spent a significant period learning against the most recent baseline policy, $\bphi^{-i}_{t^i_{m+1}}.$ In other words, the event $B_k$ should capture the event that, for suitably large $W \in \nn$, one has that $\bphi_{t^i_{m+1} - W} = \dots = \bphi_{t^i_{m+1}}$, so that player $i$ would have spent the last $W$ time steps learning against the most recent joint policy.\footnote{A related consideration here is that player $i$'s Q-factor estimates at time $t^i_{m+1} - W$ are not too far from $Q^{*i}_{\bphi_{t^i_{m+1}}}$, which we address in \Cref{lemma:uniform-boundedness}.}
%%}
%%
%%\blue{
%%The preceding considerations now allow us to describe an issue that may arise if the equilibrium event $B_k$ is not defined carefully, via the definitions of $\{\tau^{\min}_k, \tau^{\max}_k\}_{k \geq 0}$. Continuing with the notation above, where player $i$'s $m^{th}$ exploration phase straddles $\tau^{\min}_k$, suppose another player $j$ is in a similar situation, and that $t^j_{l} < \tau^{\min}_k < t^j_{l+1}$. For concreteness, let us further assume that $t^j_l < t^i_m$ and that $t^j_{l+1} < t^i_{m+1}$, so that player $j$'s $l^{th}$ exploration starts  before player $i$'s $m^{th}$ exploration phase begins and correspondingly ends before player $i$'s $m^{th}$ exploration phase ends. Visually, this situation can be represented as in \Cref{figure:exploration-phases}. 
%%
%%Suppose now that we wish to study the Q-factors obtained by each player, conditioning on the equilibrium event $B_k$. From \Cref{figure:exploration-phases}, one can see that the $m^{th}$ exploration phase (EP) for player $i$ overlaps to a significant extent with the $l^{th}$ EP for player $j$. We remark that each players Q-factors are a function of the state-action trajectory $\{ ( x_t, \ba_t ) : t= t^j_l, t^j_l + 1, \dots, t^i_{m+1} \}$. 
%%}

\blue{
Any useful definition of $\{ B_k \}_{k \geq 0}$ must be \emph{self-reinforcing}, in the sense that $\P ( B_{k+L} | B_k )$ should be controllable by appropriate choice of hyperparameters. In particular, the most natural way to approach this is by attempting to control the conditional probability that players approximately recover their equilibrium Q-functions given that the equilibrium event occurred. (That is, one wishes to control the conditional probability that, given $B_k$,
\[
\widehat{Q}^i_{t^i_{m+1}} \approx Q^{*i}_{\bphi^{-i}_{t^i_{m+1}}},
\]
for exploration phase indices $m$ belonging to some relevant range.)
}

\blue{
One issue that arises in the unsynchronized case, but not in the synchronized case, has to do with the confounding effect of conditioning on the equilibrium event $B_k$. In the unsynchronized setting, the conditioning event $B_k$ invariably carries information about both the past (before $\tau^{\min}_k$) and future (after $\tau^{\min}_k$) of the state-action trajectory $\{ (x_t, \ba_t ) \}_{t \geq 0}$. Moreover, this additional information need not be advantageous.}
\blue{
For an illustration, consider the exploration phase schedule presented in \Cref{figure:exploration-phases}, below. In this diagram, we consider two players, $i$ and $j$, who have exploration phases (EPs) straddling $\tau^{\min}_k$. That is, we have both $t^i_m < \tau^{\min}_k < t^i_{m+1}$ and $t^i_l < \tau^{\min}_k < t^i_{l+1}$. The conditioning event $B_k$ implies that player $j$ does not change its policy at time $t^j_{l+1}$. However, this sub-event carries information about player $j$'s Q-factor estimates at time $t^j_{l+1}$, which in turn carry information about the state-action trajectory $\{ ( x_t, \ba_t ) : t^j_l \leq t \leq t^j_{l+1} \}$. Further, $B_k$ implies that player $i$ does not change its policy at time $t^i_{m+1}$, which similarly  conveys information about the state-action trajectory $\{ ( x_t, \ba_t ) : t^i_m \leq t \leq t^i_{m+1} \}$. Continuing this way (chaining overlapping exploration phases from one player to the next), one sees that conditioning on $B_k$ carries substantial information about the state-action trajectory both before and after $\tau^{\min}_k$, which complicates the task of making statements about the evolution of Q-factor iterates, which depend on the state-action trajectory.
}

\blue{
At first sight, the situation above seems advantageous, since conditioning on $B_k$ seems to indicate that state-action trajectories consistent with an equilibrium event are more likely in future periods. However, this first impression need not be accurate, and the situation is a bit more subtle. Indeed, making uniform lower bounds on the conditional probability of remaining at equilibrium is difficult, and pathological histories cannot be ruled out.
}
\blue{
For instance, suppose that the joint policy was  not  an equilibrium during the time interval $[t^j_l, t^i_{m} - 1 ]$, and it was player $i$'s switching policies from $\pi^i_{m-1}$ to $\pi^i_m$ that rendered the joint policy an equilibrium. Then, player $j$ spends one portion of its $l^{th}$ EP (in this case, the majority of its $l^{th}$ EP) learning against a non-equilibrium policy and another portion learning against an equilibrium policy. A complication becomes evident when one notices that the conditioning event $B_k$ does not indicate why player $j$ does not switch policies at time $t^j_{l+1}$: perhaps player $j$ refrained to switch policies because of unusual state-action trajectory \emph{before} time $t^i_m$ drove player $j$'s Q-factor estimates far from the Q-function associated with the joint policy at time $t^i_{m}$  or perhaps player $j$ was simply inert at time $t^j_{l+1}$ and would prefer to switch policies. In the latter case, player $i$'s Q-factors at time $t^j_{l+1}$ may be far from its Q-function for the same time, and the probability that this error will be overcome by time $t^j_{l+2}$ may be difficult to lower bound. In the former case, the unusual state-action trajectory from times $t^j_l$ to $t^i_m$ carries information about the continuation trajectory, which may cause problems when lower bounding Q-factor errors at later times. In both cases, the task of lower bounding the event $\P ( B_{k+L} | B_k )$ is far more challenging than the analogous task in the synchronized setting, and each of $B_k$, $\tau^{\min}_k$, and $\tau^{\max}_k$ must be carefully defined. 
}




{
\color{blue}
%
%
\begin{figure}
\begin{center}
\begin{tikzpicture}
% Draw horizontal axis
\draw[->] (0,0) -- (10,0) node[right] {$t$};

% Draw tick marks and label them
\foreach \x/\label in {1/{$t^j_l$}, 5/{$t^i_m$}, {6}/{$\tau^{\min}_k$}, 7/{$t^j_{l+1}$}, 9/{$t^i_{m+1}$}} {
    \draw (\x,0.1) -- (\x,-0.1) node[below] {\label};
}

% Draw overbrace
\draw [decorate,decoration={brace,amplitude=5pt},yshift=12pt] (1,0) -- (7,0) node [black,midway,yshift=10pt]  {};


% Draw underbrace
\draw [decorate,decoration={brace,amplitude=5pt, mirror},yshift=-24pt] (5,0) -- (9,0) node [below, black,midway,yshift=10pt]  {};

% Add annotations where needed
\draw (4, 0.75 ) node [above] {Player $j$'s $l^{th}$ EP};
\draw (7, -1) node [below] {Player $i$'s $m^{th}$ EP} ;

\end{tikzpicture}

\caption{A visualization of overlapping exploration phases}  \label{figure:exploration-phases}
\end{center}
\end{figure}
}






\subsubsection{Redefining Active Phases}


\blue{
Since each player's Q-factors are constructed using historical feedback data, one must account for the recent history of play when analyzing Q-iterates in the unsynchronized setting. For illustration, let us consider player $i$'s $m^{th}$ exploration phase, and let us suppose that $t^i_{m+1} \in ( \tau^{\min}_k, \tau^{\max}_k ]$, momentarily postponing how the latter interval is defined.
}

\blue{In its $m^{th}$ exploration phase, player $i$ learns from time $t^i_m$ to time $t^i_{m+1} = t^i_m + T^i_m$. During this interval, player $i$'s counterparts may have switched policies several times. Thus, if one wishes to ensure that player $i$'s Q-factor estimates at time $t^i_{m+1}$ accurately reflect the prevailing environment, which is determined by $\bphi^{-i}_{t^i_{m+1}}$, then the conditioning event $B_k$ should guarantee that player $i$ spent a significant period learning against the most recent baseline policy, $\bphi^{-i}_{t^i_{m+1}}.$ In other words, the event $B_k$ should capture the event that, for suitably large $W \in \nn$, one has that $\bphi_{t^i_{m+1} - W} = \dots = \bphi_{t^i_{m+1}}$, so that player $i$ would have spent the last $W$ time steps learning against the most recent joint policy.\footnote{A related consideration here is that player $i$'s Q-factor estimates at time $t^i_{m+1} - W$ are not too far from $Q^{*i}_{\bphi_{t^i_{m+1}}}$, which we address in \Cref{lemma:uniform-boundedness}.}
}




\blue{
To properly account for the recent history of play in our definition of the equilibrium event, we define the sequences $\{ \tau^{\min}_k\}_{k \geq 0}$, $\{ \tau^{\max}_k \}_{k \geq 0}$.
}

\blue{
\begin{definition}   \label{def:active-phases}
Let $\tau^{\min}_0 = \tau^{\max}_0 := 0$. For $k \geq 0$, define
\begin{align*}
\tau^{\min}_{k+1} 	&:= \inf \{ t^i_n : t^i_n > \tau^{\max}_{k} , i \in \NN, n \geq 0 \} \\
%%% old multi-line version:
%%
\tau^{\max}_{k+1}	&:= \inf {\big \{ } t \geq \tau^{\min}_{k+1} :  \forall \, i \in \NN, \exists \, n \in \nn \text{ s.t. } t^i_{n} \in [\tau^{\min}_{k+1} , t ],   \\  	
					&\qquad \quad \qquad \quad \qquad \text{ and } \inf \{  t^i_{\bar{n}} > t : i \in \NN, \bar{n} \in \nn \} \geq t + T/N { \big \}},
\end{align*}
where $T$ is the constant appearing in \Cref{assumption:exploration-phases}.
\end{definition}
}


\blue{
The intervals $[ \tau^{\min}_k , \tau^{\max}_k ]$ represent active phases, during which players may change their policies. In the special case of synchronization, where $T^i_k = T^j_k \geq T/N$ for all players $i$ and $j$ and for all indices $k \geq 0$, these definitions yield $\tau^{\min}_k = \tau^{\max}_k = t_k$ for $k \geq 0$, coinciding with the synchronized analysis described in \Cref{ss:proof-with-synchronization}. 
}

\blue{
The properties of these active phases are described in greater detail in \Cref{lemma:active-phases} and in the discussion after its proof. For the moment, we summarize some especially useful consequences of \Cref{def:active-phases} below:
\begin{itemize}
	\setlength \itemsep{1pt}
	\item[(1)] No policy updates occur in $( \tau^{\max}_k, \tau^{\min}_{k+1} )$.
	\item[(2)]  {Each agent has at least one opportunity to switch policies during $[\tau^{\min}_{k+1}, \tau^{\max}_{k+1}]$.}  % trim or edit, if needed 
%	\item[(3)]  At time $\tau^{\max}_{k+1}$, no agent finishes its current ongoing exploration phase in the next $T/N$ stage games.
	\item[(3)]  For each $k \geq 0$, $\tau^{\min}_{k+1} \geq \tau^{\max}_k + T/N$. 
	\item[(4)] {Any player has at most $R+1$ opportunities to switch its policy during $[ \tau^{\min}_k , \tau^{\max}_k ] $.} % trim or edit, if needed 
\end{itemize}
}

\vspace{5pt}

\blue{
Since $\tau^{\min}_{k+1}$ is the first time after $\tau^{\max}_k$ at which any agent has the opportunity to switch its policy, the first and third items above offers a means by which $B_k$ can be self-reinforcing: given $B_k$, one is guaranteed that each player $i$ spends at least $T/N$ stages learning against the unchanging policy $\bphi^{-i}_{\tau^{\max}_k}$. Indeed, other formulations of $\tau^{\min}_k$ and $\tau^{\max}_k$ were considered, but simpler alternatives could not yield a meaningful analog of item (3). 
}

\vspace{5pt}

\blue{
The extent to which $\P ( B_{k+L} | B_k )$ can be controlled depends on the conditional probability that, given $B_k$, agents learn their equilibrium Q-factors approximately correctly. This, in turn, depends on the specific Q-learning update used and the length of time spent learning against outdated environments. If an agent uses decreasing step-sizes and has a relatively long exploration phase, then by the time play first arrives at equilibrium, this player's learning rates will be very small and the player will have spent the majority of its exploration phase learning against older, possibly irrelevant joint policies. These considerations lead to the utilization of constant learning rates in Algorithm~\ref{algo:main}. Constant learning rates allow for an agent to quickly change its Q-factors in response to a change in the joint policy. 
}

\vspace{11pt}

\blue{
\noindent \textbf{Remark:} Note that the sequences $\{ \tau^{\min}_{k} \}_{k \geq 0}$ and $\{ \tau^{\max}_{k} \}_{k \geq 0}$ are merely analytical devices, and the properties outlined in the list above are consequences of the analytical definitions of these objects. In particular, we wish to stress that players do not observe whether or not they are in an active phase (that is, whether the current time $t \in [ \tau^{\min}_k , \tau^{\max}_k ]$ for some $k$) or whether they are in an inactive phase  (that is, whether the current time $t \in [ \tau^{\max}_k , \tau^{\min}_{k+1} ]$ for some $k$). Our use of the sequences  $\{ \tau^{\min}_{k} \}_{k \geq 0}$ and $\{ \tau^{\max}_{k} \}_{k \geq 0}$ should not be misunderstood as coordination on the part of the players: there is no agreement between players, either implicit or explicit, to refrain from updating one's policy during an inactive window. This convenient fact is simply a result of \Cref{def:active-phases}. 
}

==> supporting-lemmas.tex <==


